Private Hierarchical Clustering in Federated Networks

Analyzing structural properties of social networks, such as identifying their clusters or finding their most central nodes, has many applications. However, these applications are not supported by federated social networks that allow users to store their social links locally on their end devices. In the federated regime, users want access to personalized services while also keeping their social links private. In this paper, we take a step towards enabling analytics on federated networks with differential privacy guarantees about protecting the user links or contacts in the network. Specifically, we present the first work to compute hierarchical cluster trees using local differential privacy. Our algorithms for computing them are novel and come with theoretical bounds on the quality of the trees learned. The private hierarchical cluster trees enable a service provider to query the community structure around a user at various granularities without the users having to share their raw contacts with the provider. We demonstrate the utility of such queries by redesigning the state-of-the-art social recommendation algorithms for the federated setup. Our recommendation algorithms significantly outperform the baselines which do not use social contacts and are on par with the non-private algorithms that use contacts.

==> chapters/abstract.tex <==
% Analyzing structural properties of graphs, such as identifying the clusters in them or finding their most central nodes, has many practical applications. However, privacy concerns arise when third-party services perform such analyses on graphs that contain privacy-sensitive relationships between users (e.g., their social links). In this paper, we present the first work to compute hierarchical cluster trees to answer such queries on {\em federated} graphs with differential privacy. In our setup, no third-party service is trusted to protect the privacy of users---we design algorithms in the local differential privacy regime. We provide theoretical bounds on the quality of our cluster trees as measured by a popular cost function vs. privacy loss. On real-world public graph datasets, we empirically show that our private hierarchical cluster trees have high quality for reasonable privacy parameters. Further, we demonstrate the utility of our private hierarchical cluster trees by redesigning the state-of-the-art privacy-violating social recommendation algorithms for the federated setup with an LDP guarantee. Our recommendation algorithms significantly outperform the private non-social baselines and are on par with the privacy-violating social baselines.

Analyzing structural properties of social networks, such as identifying their clusters or finding their most central nodes, has many applications. However, these applications are not supported by federated social networks that allow users to store their social links locally on their end devices. In the federated regime, users want access to personalized services while also keeping their social links private. In this paper, we take a step towards enabling analytics on federated networks
with differential privacy guarantees about protecting the user links or contacts in the network. Specifically, we present the first work to compute hierarchical cluster trees using local differential privacy. Our algorithms for computing them are novel and come with theoretical bounds on the quality of the trees learned. The private hierarchical cluster trees enable a service provider to query the community structure around a user at various granularities without the users having to share their raw contacts with the provider. We demonstrate the utility of such queries by redesigning the state-of-the-art social recommendation algorithms for the federated setup. Our recommendation algorithms significantly outperform the baselines which do not use social contacts and are on par with the non-private algorithms that use contacts.


==> chapters/implementation.tex <==
\paragraph{Experimental Setup}
%\label{sec:implementation}
We use $3$ real-world networks which are commonly used for evaluating recommender systems~\cite{wang2018collaborative,shepitsen2008personalized,ma2011recommender,qin2017CCS}~\footnote{https://grouplens.org/datasets/hetrec-2011/}.
%\newtext{We additionally evaluate on $3$ social networks (\facebook, \twitch, \advogato) which contain only social links, without item ratings.}
%\prateek{Cite something, and why only 3}
%Our graph sizes vary from $1503$ to $2848$ vertices and from $6350$ to $25185$ edges, respectively.
We detail the networks in Table~\ref{tab:datasets}.
\newtext{We use privacy budget values of $\epsilon\in\{0.5, 1.0, 2.0\}$ as they have been used in the prior work for both centralized as well as the local differential privacy setup~\cite{hsu2014differential,qian2014KDD,abadi2016deep}.}
% \prateek{You may want to say that these values are used in prior work. I am not quite sure why they are considered reasonable and by whom. For instance, will they be reasonably next year too?}
% 
%
% All our experiments are run on a server with 32GB RAM, AMD Ryzen 7 2700X 8-core processor and a
% GeForce RTX 2070 with 8GB RAM.
%
We have two tunable parameters: the number of bins $\numbins$ and the convergence criteria for MCMC in \localalgo. The $\numbins$ is chosen such that it minimizes the noise in the final degree vector as well as it minimizes the number of collisions in the degree vector calculation. A higher $\numbins$ minimizes the collisions but incurs more noise on aggregate and vice versa. Previous work has shown that the value of $\numbins$ is usually small and it depends on the graph structure. 
% Under a set of assumptions, prior work provides a formula to compute $\numbins$ but we observe that even under those assumptions the formula results in negative values for $\numbins$ for some graphs.
\newtext{We therefore heuristically choose $\numbins=\lfloor \log{n}\rfloor$ as it is not too low for not capturing any edge information (see Section~\ref{sec:approach}) and not too high so that we might end up adding a lot of noise (see Section~\ref{sec:prob_setup}). If we substitute this $K$ value in our utility bound for \dplocalalgo in Theorem~\ref{thm:t8}, we get a loss scaling with $\frac{\log{n}}{n\cdot\epsilon}$. Further, our values of $K$ agree with the ones used in the prior work~\cite{qin2017CCS}}. 
% \prateek{Please don't dismiss the concern like this. Prior work is broken. Plus, its analysis is completely different from yours.}
% \prateek{Be careful with surprising the reader here. Does this affect the analysis or guarantee? What gets affected with k?}
%to strike an intuitive balance.
%
We use a convergence criteria that is similar to the ones used by prior works in the centralized setting for their MCMC algorithm~\cite{qian2014KDD,clauset2008Nature}.

%We continuously examine the average $\dasgupta$ cost over a window of size $65536$ iterations. If the average difference across consecutive windows is in the interval of $[-0.05n, 0.05n]$ then we say our chain has converged. 


% Finally, we normalize the inputs before training which is done in practice.


==> figures/fig-sp-dist-hct.tex <==
\begin{figure*}[h]
% \centering
\scalebox{0.5}{
\begin{tikzpicture}
	\begin{axis}[
	    ylabel = $Mean_{u_t}(SP_{m})$,
	    label style={font=\Huge},
        tick label style={font=\Huge},
        title={\lastfm},
        title style={font=\Huge},
	]
% 	\addplot+[scatter,only marks,scatter src=y]
    \addplot+[scatter,only marks,scatter src=y, mark size=0.1 em]
		table[x=ind, y=dist, col sep=comma] {figures/data-rec/sp_dist_lastfm.csv};
	\end{axis}
\end{tikzpicture}
}
%
\scalebox{0.5}{
\begin{tikzpicture}
	\begin{axis}[
	    ylabel = {},
	    xlabel = {},
	   % ylabel = avg. shortest path distance,
	   % xlabel = index of community (0 is the closest),
	    label style={font=\Huge},
        tick label style={font=\Huge},
        title={\delicious},
        title style={font=\Huge},
	]
	\addplot+[scatter,only marks,scatter src=y, mark size=0.1 em]
		table[x=ind, y=dist, col sep=comma] {figures/data-rec/sp_dist_delicious.csv};
	\end{axis}
\end{tikzpicture}
}
%
\scalebox{0.5}{
\begin{tikzpicture}
	\begin{axis}[
	   % ylabel = avg. shortest path distance,
	   % xlabel = index of community (0 is the closest),
	    label style={font=\Huge},
        tick label style={font=\Huge},
        title={\douban},
        title style={font=\Huge},
        xtick={0,1000,2000,3000}
	]
	\addplot+[scatter,only marks,scatter src=y, mark size=0.1 em]
		table[x=ind, y=dist, col sep=comma] {figures/data-rec/sp_dist_douban.csv};
	\end{axis}
\end{tikzpicture}
}
\begin{minipage}{.45\textwidth}
    index of $Mean_{u_t}(SP_{m})$ (0 is the closest)
\end{minipage}
%
\caption{ The average shortest path distance on Y-axis, at index $i$ on X-axis, is computed on the $i^{th}$ set of closest users of size $10$. For all three datasets, the set of users at the first few indices have lower distances compared to the higher indices. Further, there is a rising trend of average shortest path distances for \lastfm and \douban HCT and not so much for \delicious. This reflects the better performance of \dplocalalgo based recommendations in \lastfm and \douban than in \delicious. }
\label{fig:sptrends}
\end{figure*}

